Evaluating the Evaluation of Diversity in Natural Language Generation

Despite growing interest in natural language generation (NLG) models that produce diverse outputs, there is currently no principled method for evaluating the diversity of an NLG system. In this work, we propose a framework for evaluating diversity metrics. The framework measures the correlation between a proposed diversity metric and a diversity parameter, a single parameter that controls some aspect of diversity in generated text. For example, a diversity parameter might be a binary variable used to instruct crowdsourcing workers to generate text with either low or high content diversity. We demonstrate the utility of our framework by: (a) establishing best practices for eliciting diversity judgments from humans, (b) showing that humans substantially outperform automatic metrics in estimating content diversity, and (c) demonstrating that existing methods for controlling diversity by tuning a "decoding parameter" mostly affect form but not meaning. Our framework can advance the understanding of different diversity metrics, an essential step on the road towards better NLG systems.

==> figures/d_tree.tex <==
\forestset{
  direction switch/.style={ %grow=right,
    for tree={edge+=thick}, % , font=\sffamily},
    where level>=1{folder, grow'=0}{for children=forked edge},
    where level>=2{}{draw},
  },
}

\centering
\begin{forest}
  % forest preamble: determine layout and format of tree
  direction switch
  [diversity
    [form
    %   [morphology
    %   ]
      [syntactic
      ]
      [lexical
        [register]
        [...]
      ]
      [...
      ]
    ]
    [content
      [sentiment
      ]
      [relevance
      ]
      [...
      ]
    ]
  ]
\end{forest}


==> figures/fig1_old.tex <==
% \usepackage{amsfonts}
% \usepackage{booktabs}
% \usepackage{siunitx}
% \usepackage{tabularx}
\newcolumntype{s}{>{\hsize=.5\hsize}X}

% \begin{tabular}{ll} 
\begin{tabularx}{\columnwidth}{|s|s|}
    % \multicolumn{2}{l}{\textbf{Reddit comment:}} \\
    
    \multicolumn{2}{c}{\resizebox {\columnwidth} {!}{\includegraphics{ {figures/fig_test_2_resp_gen_gold_kde.png}}}} \\
    
    \multicolumn{2}{c}{\textbf{So what did I miss in the first 20 minutes?}} \\
    \multicolumn{2}{l}{}  \\
    \hline
    % \textbf{\textcolor{blue}{Response set A}} & \textbf{\textcolor{orange}{Response set B}} \\    \textbf{\textcolor{blue}{Diverse content}} & \textbf{\textcolor{orange}{Constant content}} \\
    \textbf{\textcolor{blue}{Set A}} & \textbf{\textcolor{orange}{Set B}} \\
    \hline
      Pretty much everything. &    Not much.\\
      \hline
      Nothing, really. &    It was pretty dull.\\
      \hline
      You won't believe what happened! &   Blah, you didn't miss anything.\\
      \hline
      Why do you even care? &      Not anything that important.\\
      \hline
      What were you doing that was more important than this? &    Very little, it was uneventful.\\
    \hline
    \multicolumn{2}{l}{} \\

% \end{tabular}
\end{tabularx}

==> figures/test_flow_old.tex <==
% \usepackage{tikz}
% \usetikzlibrary{arrows.meta}

% % Drawing part, node distance is 1.5 cm and every node
% % is prefilled with white background
\begin{tikzpicture}[node distance=1.5cm,
every node/.style={fill=white, font=\sffamily}, align=center]

\tikzset{
% 	>={Latex[width=2mm,length=2mm]},
	% Specifications for style of nodes:
	base/.style = {rectangle, rounded corners, draw=black,
		minimum width=4cm, minimum height=1cm,
		text centered, font=\sffamily},
	io/.style = {base, fill=red!30},
	block/.style = {base, fill=blue!30},
	line/.style={
    draw,rounded corners=3mm, -latex,
    }
}

% Specification of nodes (position, etc.)
\node (div_param) [io] {Diversity Parameter};
\node (context) [io, right of=div_param, right=2cm] {Context};
\node (tester) [block, below of=div_param, right=1cm] {Tester};
\node (metric) [block, below of=tester, below=.1cm] {Metric under test};
\node (rho) [block, below of=metric, below=.1cm] {$\rho$};
\node (score) [io, below of=rho, below=.05cm] {Test Score};

% Specification of lines between nodes specified above
% with additional nodes for description 
\path[line]     (div_param.290) |-  (tester);
\path[line]     (context) |- (tester);
\path[line]     (tester) -- node [right, align=right]{response set}(metric);
\path[line]     (metric) -- node [right, align=right]{metric score}(rho);
\path[line]     (div_param.250) |- (rho);
\path[line]     (rho) -- (score);

\end{tikzpicture}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
